Multi-species MCTDHF for gate simulations in multi-qubit hardware

Gate fidelities of quantum hardware are usually estimated with few-level models, in which the level structure and the couplings between the qubits are fixed in advance. Here, we apply the multi-species multiconfiguration time-dependent Hartree-Fock (MCTDHF) method to gate calculations at the hardware level, where the spectrum and the couplings instead follow from the dynamics of the system. Each qubit is treated as a separate species with its own time-dependent orbitals. As a test case, we engineer $\sqrt{i\mathrm{SWAP}}$ gates in a one-dimensional register of four anharmonic wells. First, we simulate the system with one electron per well and validate the method against an untruncated propagation of the register. We also construct a gate between the two outermost qubits from circuits of nearest-neighbor gates. The fidelity of these circuits is not reliably predicted by the individual gates, so the circuits have to be propagated as a whole. We then simulate the system with three spin-polarized electrons per well, where the gates fail through leakage out of the state $|11\rangle$. A calculation with too few orbitals misses this leakage and reports a high-fidelity gate instead. Capturing the leakage requires a large number of orbitals, which a multilayer form of the ansatz makes feasible. These results show that the method is a suitable tool for designing gates in multi-qubit hardware, where the errors of a gate are not confined to the computational subspace of the qubits it acts on.

==> main-labels.tex <==
% Labels from main.aux, generated for the arXiv build (replaces xr).
\newlabel{sec:intro}{{I}{1}{}{}{}}
\newlabel{sec:mctdhf}{{II}{2}{}{}{}}
\newlabel{sec:ansatz}{{II\,A}{2}{}{}{}}
\newlabel{eq:ansatz}{{1}{2}{}{}{}}
\newlabel{eq:bexp}{{2}{2}{}{}{}}
\newlabel{sec:eom}{{II\,B}{3}{}{}{}}
\newlabel{eq:ham}{{3}{3}{}{}{}}
\newlabel{eq:ci}{{4}{3}{}{}{}}
\newlabel{eq:orb}{{5}{3}{}{}{}}
\newlabel{sec:discretization}{{II\,C}{3}{}{}{}}
\newlabel{eq:bdot}{{6}{3}{}{}{}}
\newlabel{sec:stateavg}{{II\,D}{3}{}{}{}}
\newlabel{eq:densities-sa}{{7}{3}{}{}{}}
\newlabel{sec:ml}{{II\,E}{4}{}{}{}}
\newlabel{eq:sbs}{{8}{4}{}{}{}}
\newlabel{eq:ml-ansatz}{{9}{4}{}{}{}}
\newlabel{sec:ml-eom}{{II\,F}{4}{}{}{}}
\newlabel{fig:ml}{{1}{4}{}{}{}}
\newlabel{eq:ml-A}{{10}{4}{}{}{}}
\newlabel{eq:ml-B}{{11}{4}{}{}{}}
\newlabel{eq:ml-rho}{{12}{4}{}{}{}}
\newlabel{sec:application}{{III}{5}{}{}{}}
\newlabel{sec:sys-fourwell}{{III\,A}{5}{}{}{}}
\newlabel{eq:h1}{{13}{5}{}{}{}}
\newlabel{eq:well}{{14}{5}{}{}{}}
\newlabel{eq:ham-fourwell}{{15}{5}{}{}{}}
\newlabel{sec:gate-engineering}{{III\,B}{5}{}{}{}}
\newlabel{sec:op-points}{{III\,B\,1}{5}{}{}{}}
\newlabel{sec:td-opt}{{III\,B\,2}{6}{}{}{}}
\newlabel{eq:time_dep_schedule}{{16}{6}{}{}{}}
\newlabel{eq:ramp}{{17}{6}{}{}{}}
\newlabel{sec:fidelity}{{III\,B\,3}{6}{}{}{}}
\newlabel{eq:fidelity}{{18}{6}{}{}{}}
\newlabel{eq:sjoj}{{19}{6}{}{}{}}
\newlabel{eq:fbar_sjoj}{{20}{7}{}{}{}}
\newlabel{eq:fidchain}{{21}{7}{}{}{}}
\newlabel{sec:longrange-test}{{III\,C}{7}{}{}{}}
\newlabel{fig:swap_decomposition}{{2}{7}{}{}{}}
\newlabel{fig:circuits}{{3}{7}{}{}{}}
\newlabel{sec:results}{{IV}{7}{}{}{}}
\newlabel{sec:fourwell}{{IV\,A}{8}{}{}{}}
\newlabel{sec:mf-res}{{IV\,A\,1}{8}{}{}{}}
\newlabel{sec:longrange-res}{{IV\,A\,2}{8}{}{}{}}
\newlabel{fig:mf}{{4}{9}{}{}{}}
\newlabel{fig:methods_fid}{{5}{10}{}{}{}}
\newlabel{sec:threewell}{{IV\,B}{11}{}{}{}}
\newlabel{fig:3e_qubit}{{6}{11}{}{}{}}
\newlabel{fig:3e_convergence}{{7}{12}{}{}{}}
\newlabel{sec:conclusions}{{V}{12}{}{}{}}
\newlabel{app:eom}{{A}{13}{}{}{}}
\newlabel{eq:sigma1}{{A1}{13}{}{}{}}
\newlabel{eq:sigma2}{{A2}{13}{}{}{}}
\newlabel{app:propagation}{{B}{13}{}{}{}}
\newlabel{app:propagation-3e}{{B\,2}{14}{}{}{}}
\newlabel{app:grid}{{B\,3}{14}{}{}{}}
\newlabel{app:exact}{{C}{14}{}{}{}}
\newlabel{tab:exact}{{I}{15}{}{}{}}

